Towards Modular LLMs by Building and Reusing a Library of LoRAs

The growing number of parameter-efficient adaptations of a base large language model (LLM) calls for studying whether we can reuse such trained adapters to improve performance for new tasks. We study how to best build a library of adapters given multi-task data and devise techniques for both zero-shot and supervised task generalization through routing in such library. We benchmark existing approaches to build this library and introduce model-based clustering, MBC, a method that groups tasks based on the similarity of their adapter parameters, indirectly optimizing for transfer across the multi-task dataset. To re-use the library, we present a novel zero-shot routing mechanism, Arrow, which enables dynamic selection of the most relevant adapters for new inputs without the need for retraining. We experiment with several LLMs, such as Phi-2 and Mistral, on a wide array of held-out tasks, verifying that MBC-based adapters and Arrow routing lead to superior generalization to new tasks. We make steps towards creating modular, adaptable LLMs that can match or outperform traditional joint training.

==> __.tex <==

c0 & 
        "adversarial\_qa\_dbert\_generate\_question", "adversarial\_qa\_dbidaf\_generate\_question", "adversarial\_qa\_droberta\_generate\_question", "app\_reviews\_generate\_review", "cot\_creak", "cot\_esnli", "cot\_esnli\_ii", "dream\_generate\_first\_utterance", "dream\_generate\_last\_utterance", "duorc\_ParaphraseRC\_title\_generation", "duorc\_SelfRC\_title\_generation", "fix\_punct", "gem\_common\_gen\_1\_1\_0", "gem\_dart\_1\_1\_0", "gigaword\_1\_2\_0", "huggingface\_xsum", "lambada\_1\_0\_0", "race\_high\_Write\_a\_multi\_choice\_question\_for\_the\_following\_article", "race\_high\_Write\_a\_multi\_choice\_question\_options\_given\_", "race\_middle\_Write\_a\_multi\_choice\_question\_for\_the\_following\_article", "race\_middle\_Write\_a\_multi\_choice\_question\_options\_given\_", "stream\_aqua", "stream\_qed", "wiqa\_what\_is\_the\_missing\_first\_step", "wmt16\_translate\_fi\_en\_1\_0\_0", "wmt16\_translate\_ro\_en\_1\_0\_0", "yelp\_polarity\_reviews\_0\_2\_0"
        \\
\midrule    
c1 & 
        "ag\_news\_subset\_1\_0\_0", "app\_reviews\_convert\_to\_rating", "app\_reviews\_convert\_to\_star\_rating", "cot\_creak\_ii", "cot\_ecqa\_ii", "cot\_gsm8k\_ii", "cot\_sensemaking\_ii", "cot\_strategyqa", "dbpedia\_14\_given\_a\_choice\_of\_categories\_", "dbpedia\_14\_given\_a\_list\_of\_category\_what\_does\_the\_title\_belong\_to", "dbpedia\_14\_given\_list\_what\_category\_does\_the\_paragraph\_belong\_to", "glue\_mnli\_2\_0\_0", "glue\_qnli\_2\_0\_0", "glue\_qqp\_2\_0\_0", "glue\_stsb\_2\_0\_0", "glue\_wnli\_2\_0\_0", "kilt\_tasks\_hotpotqa\_complex\_question", "paws\_wiki\_1\_1\_0", "qasc\_is\_correct\_1", "qasc\_is\_correct\_2", "snli\_1\_1\_0", "social\_i\_qa\_Check\_if\_a\_random\_answer\_is\_valid\_or\_not", "social\_i\_qa\_Generate\_answer", "social\_i\_qa\_Generate\_the\_question\_from\_the\_answer", "social\_i\_qa\_I\_was\_wondering", "squad\_v1\_1\_3\_0\_0", "squad\_v2\_0\_3\_0\_0", "stream\_qed\_ii", "super\_glue\_multirc\_1\_0\_2", "super\_glue\_rte\_1\_0\_2", "super\_glue\_wic\_1\_0\_2", "super\_glue\_wsc\_fixed\_1\_0\_2", "trec\_1\_0\_0", "wiki\_bio\_guess\_person", "wiki\_qa\_Is\_This\_True\_"
        \\
\midrule    
c2 & 
        "app\_reviews\_categorize\_rating\_using\_review", "cos\_e\_v1\_11\_question\_option\_description\_text", "cot\_qasc", "cot\_strategyqa\_ii", "dbpedia\_14\_pick\_one\_category\_for\_the\_following\_text", "definite\_pronoun\_resolution\_1\_1\_0", "kilt\_tasks\_hotpotqa\_final\_exam", "math\_dataset\_algebra\_\_linear\_1d\_1\_0\_0", "qasc\_qa\_with\_separated\_facts\_4", "quarel\_do\_not\_use", "quoref\_Context\_Contains\_Answer", "race\_high\_Is\_this\_the\_right\_answer", "race\_middle\_Is\_this\_the\_right\_answer", "sciq\_Direct\_Question", "sciq\_Multiple\_Choice", "sciq\_Multiple\_Choice\_Closed\_Book\_", "sciq\_Multiple\_Choice\_Question\_First", "social\_i\_qa\_Show\_choices\_and\_generate\_index", "stream\_aqua\_ii", "super\_glue\_cb\_1\_0\_2", "super\_glue\_copa\_1\_0\_2", "unified\_qa\_science\_inst", "wiki\_qa\_Decide\_good\_answer", "wiki\_qa\_Direct\_Answer\_to\_Question", "wiki\_qa\_Generate\_Question\_from\_Topic", "wiki\_qa\_Jeopardy\_style", "wiki\_qa\_Topic\_Prediction\_Answer\_Only", "wiki\_qa\_Topic\_Prediction\_Question\_Only", "wiki\_qa\_Topic\_Prediction\_Question\_and\_Answer\_Pair", "wiki\_qa\_automatic\_system", "wiki\_qa\_exercise", "wiki\_qa\_found\_on\_google"
        \\
\midrule    
c3 & 
        "adversarial\_qa\_dbert\_answer\_the\_following\_q", "adversarial\_qa\_dbert\_based\_on", "adversarial\_qa\_dbert\_question\_context\_answer", "adversarial\_qa\_dbert\_tell\_what\_it\_is", "adversarial\_qa\_dbidaf\_answer\_the\_following\_q", "adversarial\_qa\_dbidaf\_based\_on", "adversarial\_qa\_dbidaf\_question\_context\_answer", "adversarial\_qa\_dbidaf\_tell\_what\_it\_is", "adversarial\_qa\_droberta\_answer\_the\_following\_q", "adversarial\_qa\_droberta\_based\_on", "adversarial\_qa\_droberta\_question\_context\_answer", "adversarial\_qa\_droberta\_tell\_what\_it\_is", "cos\_e\_v1\_11\_aligned\_with\_common\_sense", "cos\_e\_v1\_11\_explain\_why\_human", "cos\_e\_v1\_11\_generate\_explanation\_given\_text", "cos\_e\_v1\_11\_i\_think", "cos\_e\_v1\_11\_rationale", "drop\_2\_0\_0", "duorc\_ParaphraseRC\_generate\_question\_by\_answer", "duorc\_SelfRC\_generate\_question\_by\_answer", "kilt\_tasks\_hotpotqa\_combining\_facts", "kilt\_tasks\_hotpotqa\_formulate", "kilt\_tasks\_hotpotqa\_straighforward\_qa", "natural\_questions\_open\_1\_0\_0", "trivia\_qa\_rc\_1\_1\_0", "web\_questions\_get\_the\_answer", "web\_questions\_potential\_correct\_answer", "web\_questions\_question\_answer", "web\_questions\_short\_general\_knowledge\_q", "web\_questions\_whats\_the\_answer"
        \\
\midrule    
c4 & 
        "duorc\_ParaphraseRC\_answer\_question", "duorc\_ParaphraseRC\_decide\_worth\_it", "duorc\_ParaphraseRC\_extract\_answer", "duorc\_ParaphraseRC\_generate\_question", "duorc\_ParaphraseRC\_movie\_director", "duorc\_ParaphraseRC\_question\_answering", "duorc\_SelfRC\_answer\_question", "duorc\_SelfRC\_decide\_worth\_it", "duorc\_SelfRC\_extract\_answer", "duorc\_SelfRC\_generate\_question", "duorc\_SelfRC\_movie\_director", "duorc\_SelfRC\_question\_answering", "quac\_1\_0\_0", "quoref\_Answer\_Friend\_Question", "quoref\_Answer\_Test", "quoref\_Find\_Answer", "quoref\_Found\_Context\_Online", "quoref\_Given\_Context\_Answer\_Question", "quoref\_Guess\_Answer", "quoref\_Guess\_Title\_For\_Context", "quoref\_Read\_And\_Extract\_", "quoref\_What\_Is\_The\_Answer"
        \\
\midrule    
c5 & 
        "cos\_e\_v1\_11\_description\_question\_option\_id", "cos\_e\_v1\_11\_question\_description\_option\_id", "dream\_baseline", "dream\_read\_the\_following\_conversation\_and\_answer\_the\_question", "quail\_context\_description\_question\_answer\_id", "quail\_context\_description\_question\_answer\_text", "quail\_context\_description\_question\_text", "quail\_context\_question\_answer\_description\_id", "quail\_context\_question\_answer\_description\_text", "quail\_context\_question\_description\_answer\_id", "quail\_context\_question\_description\_answer\_text", "quail\_context\_question\_description\_text", "quail\_description\_context\_question\_answer\_id", "quail\_description\_context\_question\_answer\_text", "quail\_description\_context\_question\_text", "quail\_no\_prompt\_id", "quail\_no\_prompt\_text", "race\_high\_Read\_the\_article\_and\_answer\_the\_question\_no\_option\_", "race\_high\_Select\_the\_best\_answer", "race\_high\_Select\_the\_best\_answer\_generate\_span\_", "race\_high\_Select\_the\_best\_answer\_no\_instructions\_", "race\_high\_Taking\_a\_test", "race\_middle\_Read\_the\_article\_and\_answer\_the\_question\_no\_option\_", "race\_middle\_Select\_the\_best\_answer", "race\_middle\_Select\_the\_best\_answer\_generate\_span\_", "race\_middle\_Select\_the\_best\_answer\_no\_instructions\_", "race\_middle\_Taking\_a\_test"
        \\
\midrule    
c6 & 
        "cos\_e\_v1\_11\_description\_question\_option\_text", "cos\_e\_v1\_11\_question\_description\_option\_text", "cos\_e\_v1\_11\_question\_option\_description\_id", "qasc\_qa\_with\_combined\_facts\_1", "qasc\_qa\_with\_separated\_facts\_1", "qasc\_qa\_with\_separated\_facts\_2", "qasc\_qa\_with\_separated\_facts\_3", "qasc\_qa\_with\_separated\_facts\_5", "quarel\_choose\_between", "quarel\_heres\_a\_story", "quarel\_logic\_test", "quarel\_testing\_students", "quartz\_answer\_question\_based\_on", "quartz\_answer\_question\_below", "quartz\_given\_the\_fact\_answer\_the\_q", "quartz\_having\_read\_above\_passage", "quartz\_paragraph\_question\_plain\_concat", "quartz\_read\_passage\_below\_choose", "quartz\_use\_info\_from\_paragraph\_question", "quartz\_use\_info\_from\_question\_paragraph", "quoref\_Answer\_Question\_Given\_Context", "ropes\_background\_new\_situation\_answer", "ropes\_background\_situation\_middle", "ropes\_given\_background\_situation", "ropes\_new\_situation\_background\_answer", "ropes\_plain\_background\_situation", "ropes\_plain\_bottom\_hint", "ropes\_plain\_no\_background", "ropes\_prompt\_beginning", "ropes\_prompt\_bottom\_hint\_beginning", "ropes\_prompt\_bottom\_no\_hint", "ropes\_prompt\_mix", "ropes\_read\_background\_situation", "sciq\_Direct\_Question\_Closed\_Book\_", "social\_i\_qa\_Show\_choices\_and\_generate\_answer", "wiqa\_does\_the\_supposed\_perturbation\_have\_an\_effect", "wiqa\_effect\_with\_label\_answer", "wiqa\_effect\_with\_string\_answer", "wiqa\_which\_of\_the\_following\_is\_the\_supposed\_perturbation"
        \\
\midrule    
c7 & 
        "aeslc\_1\_0\_0", "cnn\_dailymail\_3\_4\_0", "coqa\_1\_0\_0", "cot\_gsm8k", "dream\_answer\_to\_dialogue", "duorc\_ParaphraseRC\_build\_story\_around\_qa", "duorc\_SelfRC\_build\_story\_around\_qa", "gem\_e2e\_nlg\_1\_1\_0", "gem\_web\_nlg\_en\_1\_1\_0", "gem\_wiki\_lingua\_english\_en\_1\_1\_0", "multi\_news\_1\_0\_0", "wiki\_bio\_comprehension", "wiki\_bio\_key\_content", "wiki\_bio\_what\_content", "wiki\_bio\_who", "wiqa\_what\_is\_the\_final\_step\_of\_the\_following\_process", "wiqa\_what\_might\_be\_the\_first\_step\_of\_the\_process", "wiqa\_what\_might\_be\_the\_last\_step\_of\_the\_process", "wmt16\_translate\_tr\_en\_1\_0\_0"
        \\
\midrule    
c8 & 
        "anli\_r1\_0\_1\_0", "anli\_r2\_0\_1\_0", "anli\_r3\_0\_1\_0", "cosmos\_qa\_1\_0\_0", "cot\_ecqa", "cot\_sensemaking", "glue\_cola\_2\_0\_0", "glue\_mrpc\_2\_0\_0", "glue\_sst2\_2\_0\_0", "imdb\_reviews\_plain\_text\_1\_0\_0", "para\_crawl\_enes", "super\_glue\_record\_1\_0\_2", "true\_case", "wmt14\_translate\_fr\_en\_1\_0\_0", "wmt16\_translate\_de\_en\_1\_0\_0", "word\_segment"
        \\
\midrule    
c9 &
    "wiki\_hop\_original\_choose\_best\_object\_affirmative\_1", "wiki\_hop\_original\_choose\_best\_object\_affirmative\_2", "wiki\_hop\_original\_choose\_best\_object\_affirmative\_3", "wiki\_hop\_original\_choose\_best\_object\_interrogative\_1", "wiki\_hop\_original\_choose\_best\_object\_interrogative\_2", "wiki\_hop\_original\_explain\_relation", "wiki\_hop\_original\_generate\_object", "wiki\_hop\_original\_generate\_subject", "wiki\_hop\_original\_generate\_subject\_and\_object"
    \\
\bottomrule


==> extended_related_work.tex <==
\section{Extended Related Work}
\textbf{Parameter efficient fine-tuning (PEFT)}  methods facilitate efficient adaptation of LLMs without updating all the training parameters, thereby reducing the memory and computation cost \citep{zhang2023llama,lora,ansell2021composable,pfeiffer2020adapterfusion}. For example, adapter tuning \citep{houlsby2019parameter} inserts small neural modules (adapters) between the layers of the basic model. Prefix tuning \citep{liu2021p} and Prompt tuning \citep{lester2021power} add some tunable vectors to the input or hidden layer of the base model. These models can achieve comparable performance to full-finetuning while only using less than 1\% training parameters. \citep{lora} propose a method named \texttt{LoRA}, which parameterizes incremental weights $\Delta$ as a low-rank matrix. IA3~\citep{liu2022few} focuses on scaling the activations.

\textbf{Multi-task learning} (MTL) aims to learn a model with enhanced generalization across seen and unseen tasks~\cite{caruana1997multitask}. Traditional MTL techniques involve training on a joint dataset of all tasks, potentially leading to performance degradation due to cross-task interference~\cite{zhao2018modulation}. To address this, various approaches have been proposed for partitioning learnable parameters into shared and task-specific components~\cite{ding2023mitigating,strezoski2019many,bragman2019stochastic,zaremoodi2018adaptive,wallingford2022task}. Some methods advocate for completely independent training of domain-specific models that can be full models or PEFT experts. In this spirit~\cite{vu2021spot} propose SPoT -- a few-shot transfer approach in which a set of task specific soft prompts form an MTL system. When adapting to a new task, a most suitable soft prompt is retrieved and fine-tuned for this task. In contrast to SPoT, in this work we ensemble multiple LoRA modules for both zero- and few-shot transfer, as well as propose clustering techniques that can further boost performance of a PEFT library based MTL system. In a similar spirit~\citet{li2022branch,don2022cold,gururangan2023scaling} train full expert models per domain while periodically merging their parameters into a unified model atop a strong base model. Independent expert training offers benefits such as gradient synchronization and data privacy, while merging step can enable cross-expert transfer and results into a single model alleviating the need for expert routing. In this work, we take the path of independent expert training, while exploring routing techniques beyond simple uniform averaging.

\textbf{Mixture of experts} (MoEs), when coupled with sparse routing, are notable for augmenting model capacity with minimal computational overhead \cite{fedus2021switch}. Recent works by \citet{caccia2023multihead,ponti2022combining} showcase the effectiveness of densely routed PEFT experts trained end-to-end with an expert library for MTL fine-tuning. In contrast, we apply dense routing atop of \textit{independently} trained domain experts. For expert aggregation, we employ parameter-space weighted expert averaging~\cite{wortsman2022model} with weights induced by a learned router, a technique akin to those in previous works~\cite{ostapenko2023case,zadouri2023pushing}. 

\textbf{Model ensembling} techniques aim to enhance model robustness and generalization by integrating multiple distinct models. Parameter space averaging of independent models~\cite{frankle2020linear,wortsman2022model} serves as an efficient ensembling method for full models~\cite{ilharco2022editing,ainsworth2022git} and PEFT adapters~\cite{zhang2023composing}, requiring only a single forward pass through the model, unlike output space ensembling~\cite{dietterich2000ensemble,breiman1996bagging}, that requires as many forward passes as ensembled models.  On a similar note, \citet{pfeiffer2020adapterfusion} proposed ensembling of bottleneck style adapters with the subsequent fine-tuning step. We emphasize, that in contrast to the existing works that usually study parameter merging of a relatively small number of models (typically $\leq$ 10), here we tackle the problem of ensembling of over 200 experts.



\textbf{Clustering techniques} have been widely employed to bolster LM training and decrease task interference~\cite{fifty2021efficiently}. These methods include clustering on tf-idf and neural embeddings, k-means clustering with balanced linear assignment, and soft clustering with GMMs \citep{gross2017hard, chronopoulou2023adaptersoup, chronopoulou2021efficient, gururangan2023scaling, duan2021enslm, caron2018deep} to name a few. Notably, recent research by \citet{zhou2022efficiently} observed the potential of PEFT adapter parameters as effective task embeddings for clustering purposes, a concept we leverage in this work. A similar observation, but with regards to task gradients has been made by~\citet{vu2020exploring}.

\paragraph{Library of composable experts} has been envisioned in several previous works. For instance, \citet{beck2021adapterhub,poth2023adapters} orchestrated a framework for assembling diverse PEFT adapters, offering flexibility in both training and inference. In contrast to this work, they do not consider combining independently trained adapters. On a related note \citet{kang2023self} study self-specialization of LoRa experts, conceptualizing but not materializing a dynamic library of such experts for on-the-fly selection. Finally, and most related to this work, \citet{huang2023lorahub} build LoRaHub, which is a library of task specific LoRa adapters that can be combined for few-shot downstream generalization. While conceptually similar, our work surpasses the scope of LoRaHub, that does not extend beyond few-shot task adaptation with non-gradient based optimization techniques.





==> sec_summary.tex <==

\section{Summary}

Main take-aways:
\begin{itemize}
\item Model-based clustering (MBC) / Task-Vector Clustering (have ties to tv paper), better to minimize interference for SMALL models.
\item Outperform other types of clustering for both 0-shot and few-shot evaluation.
\item For few-shot, adapters trained w. MBC are more re-usable
\item For 0-shot, MBC trains mergeable adapters? (0-shot merging)
\end{itemize}

Related Works:
\begin{itemize}
\item \cite{zhou2022efficiently} Efficiently tuned parameters are task embeddings 
\item check related works for clustering
\end{itemize}

Main experiments:
\begin{itemize}
\item Plot w task-wise transfer vs joint transfer wrt LoRA embedding similarity: more transfer with similar adapters
\item Flan -- 263 experts - 10 held-out tasks + code / mmlu (phi-2), generalization on 12 test held-out tasks on SNI
\item Test Phi-2 (AND Gpt-Neo 1.3B) on the Flan to get a sense of how things change (how long does it take on llama2-7b -- pythia-410m? check open-llm leaderboard)
\item Result on the test set of the training tasks: MBC experts lead to higher in-distribution performance than joint and per-task experts
\item "good" downstream 0-shot result for Phi-2
\item low-priority (T0 benchmark -- 38 experts - 11 held-out tasks (t5-xl-lm))
\item Merging with Uniform merging or Ties merging (Lucas has a PR on that)
\end{itemize}

Baselines:
\begin{itemize}
\item Full fine-tuning
\item LoRA shared fine-tuning
\item Poly, MHR, MoPE, Adapter-Soup, few-shot and 0-shot (look results in the Cohere paper -- figure out differences)
\end{itemize}

Ablations that we need:
\begin{itemize}
\item Train shared adapter / full fine-tuning
\item Transfer matrix vs. LoRA parameters
\item Different types of clustering: (random clustering, tf-idf, embedding based)
\item (low-pri:) Soft vs Hard K-Means ?
\item Try different number of clusters -- optimal amount of clusters?
\item KMeans on the similarity vs KMeans on the embeddings, DB-Scan type of clustering
\item (Optional:) Different type of adapters? Does it work better/worse with soft-prompts?
\end{itemize}

Comparisons with Polytropon?
\begin{itemize}
\item Compare task similarity between routings inferred by Polytropon with SVD based embeddings.
\end{itemize}

